Machine Theory of Mind for Autonomous Cyber-Defence

Intelligent autonomous agents hold much potential for the domain of cyber-security. However, due to many state-of-the-art approaches relying on uninterpretable black-box models, there is growing demand for methods that offer stakeholders clear and actionable insights into their latent beliefs and motivations. To address this, we evaluate Theory of Mind (ToM) approaches for Autonomous Cyber Operations. Upon learning a robust prior, ToM models can predict an agent's goals, behaviours, and contextual beliefs given only a handful of past behaviour observations. In this paper, we introduce a novel Graph Neural Network (GNN)-based ToM architecture tailored for cyber-defence, Graph-In, Graph-Out (GIGO)-ToM, which can accurately predict both the targets and attack trajectories of adversarial cyber agents over arbitrary computer network topologies. To evaluate the latter, we propose a novel extension of the Wasserstein distance for measuring the similarity of graph-based probability distributions. Whereas the standard Wasserstein distance lacks a fixed reference scale, we introduce a graph-theoretic normalization factor that enables a standardized comparison between networks of different sizes. We furnish this metric, which we term the Network Transport Distance (NTD), with a weighting function that emphasizes predictions according to custom node features, allowing network operators to explore arbitrary strategic considerations. Benchmarked against a Graph-In, Dense-Out (GIDO)-ToM architecture in an abstract cyber-defence environment, our empirical evaluations show that GIGO-ToM can accurately predict the goals and behaviours of various unseen cyber-attacking agents across a range of network topologies, as well as learn embeddings that can effectively characterize their policies.

==> inc/reportincs.tex <==
%--------------------------------------
% Report specific packages
% \usepackage[numbers]{natbib}
% \usepackage{graphicx,subfig}
% \usepackage[T1]{fontenc}
% \usepackage{changepage}
% \usepackage{tcolorbox}
% \usepackage{todonotes}
% \usepackage{hyperref}
% \usepackage{datatool}
% \usepackage{graphicx}
% \usepackage{multirow}
% \usepackage{thmtools}
% \usepackage{minted}
% \sloppy % to prevent margin overflow
% % ----------------------------------
% % New commands
% \input{inc/newcommands}
% \newcommand{\WP}{Wolpertinger\xspace}
% \newcommand{\report}{report\xspace}
% \newcommand{\Z}{\mathcal{Z}}
% \newcommand{\R}{\mathcal{R}}
% \newcommand{\state}{s}
% %\renewcommand{\state}{s}
% \theoremstyle{definition}
% \setcitestyle{citesep={;}}

==> sections/background.tex <==
\section*{Background} \label{sec:background}

\subsection*{Partially Observable Markov Games} \label{sec:background:pomg}

The agents discussed in
this report are types of
\emph{partially observable Markov games} (POMGs).
%
Unlike in (fully observable) Markov Games,
which are also known as stochastic games \cite{shapley1953stochastic},
within a POMG the full state of the environment is hidden from all players.
%
As a result the players only have access to their own limited observations.
%
For example, a cyber-attacking agent will typically be unable to observe
the complete layout of the network and all the services running on each node.
%
Similarly, a cyber-defence agent will rarely be able to observe the
full state of the network, given the computational overhead
that would be required in relaying all of this information to the cyber-defence
agent at every time-step.

Formally, a Markov game $\M$
is defined as a tuple $(n, \states, \actions, \transition, \rewards, \gamma)$,
consisting of:
%
\begin{itemize}

    \item The number of players (agents) $n$.

    \item A finite state space $\states$.

    \item A joint action space $(\actions_1 \times ... \times \actions_n)$ for each state $\state \in \states$, with $\actions_p$ being the number of actions available to player $p$ within a state $\state$.

    \item A state transition function $\transition : \states_t \times \actions_1 \times ... \times \actions_n \times \mathcal{\states}_{t+1} \rightarrow [0,1]$, returning the probability of transitioning from a state $\state_t$ to $\state_{t+1}$ given an action profile $\action_1 \times ... \times \action_n$.
    %
    Here, each action $\action_p$ belongs to the set of actions available to player $p$: $\action_p \in \actions_p$.
    %
    Therefore, $\transition$ captures the state transition probability (ranging from and including $0$ to $1.0$) for transitioning from
    any given state $\state$ to a next state $\state'$ for every possible joint-action profile $\action_1 \times ... \times \action_n$.

    \item A set of discount rates $\gamma$, where $\gamma_p$ defines player $p$'s
    preference over immediate and future rewards within the decision-making process.
    %
    Larger values for $\gamma$ define a preference for long-term rewards.

    \item A set of reward functions $\mathcal{\rewards}$. For each player $p$, $\mathcal{\rewards}$ contains a reward function:
    $\mathcal{\rewards}_p : \mathcal{\states}_t \times \mathcal{\actions}_1 \times ... \times \mathcal{\actions}_n \times \mathcal{\states}_{t+1} \rightarrow \rats$,
    that returns a reward $r_p$ \cite{shapley1953stochastic}.
\end{itemize}
%
We allow \emph{terminal states} at which the game ends.
%
Within a Markov game each state is fully-observable.
%
However, as mentioned above, in our current evaluation environment our agents will
only have partial observability.
%
Here, we have a Partially Observable Markov Game (POMG);
an extension of Markov Games that includes
$\langle \observations, \observationf \rangle$:

\begin{itemize}
    \item A set of joint observations $\observations$.
    \item An observation probability function defined as
    $\observationf_p : \states \times \actions_1 \times ... \times \actions_n \times \observations \rightarrow [0,1]$, where,
    for player $p$, a distribution over observations $\observation$ that may occur in state $\state$ is returned, given an action profile $\action_1 \times ... \times \action_n$.
\end{itemize}

\subsection*{Cyber-Defence Games} \label{sec:background:cyber-defence-games}

In this report we evaluate the ability of \tomnet architectures
to characterize agents situated within cyber-defence games.
%
Our focus is on scenarios featuring two agents,
a \red cyber-attacking agent and a \blue cyber-defence agent
(See \autoref{fig:POMG}).
%
While we shall not be training any agents using incentive based learning approaches, in \comLS{reference agents section in Methods here}
we shall evaluate the performance of rules-based Blue and Red agents.
%
The performance of each agent will be measured using:
%
i.) Their respective reward functions;
ii.) The average number of time-steps per episode, and;
iii.) Their win rate.
%
For the first metric we treat the game as zero-sum,
\ie $\mathcal{R}_{Red} = -\mathcal{R}_{Blue}$.
%
\begin{figure}[H]
    \centering
    \includegraphics[width=0.6\columnwidth]{img/POMG.png}
    \caption{A partially observable Markov game featuring a Red and Blue agent.}
    \label{fig:POMG}
\end{figure}

\subsection*{Machine Theory of Mind} \label{sec:background:mToM}

For \tom our task is to make predictions over a family of POMGs
%
\begin{equation}
\M = \bigcup_j \M_j,
\end{equation}
%
\ie the union over a set of POMGs $\M$,
where each $\M_j$ represents a POMG.
%
For example, the \tomnet architectures in this report are tasked with making
predictions over a range of network topologies with different node settings.
%
We also assume we have a family of agents
%
\begin{equation}
\agents = \bigcup_i \agents_i,
\end{equation}
%
with each $i$ representing an agent.
%
Using the same problem formulation as
%\cite{pmlr-v80-rabinowitz18a},
we shall associate the reward functions, discount factors,
and conditional observation functions with the agents $\agents$ rather
than the POMGs $\M$.
%
Therefore, for each POMG $\M_j$ we have a tuple
$(\states_j, \actions_j, \transition_j)$, and for each agent $\agents_i$ we have
$(\observations_i, \observationf_i, \rewards_i, \gamma_i, \pi_i)$, where
$\gamma_i$ is the discount rate, and $\pi_i$ the agent's policy belonging to agent $i$.
%
%Therefore, for each $\M_j$ we have a tuple
%$(\states_j, \actions_j, \transition_j)$.
%
%In addition we have a family of agents $A = \bigcup_i A_i$,
%where each $A_i = (\observations_i, \observationf_i, \rewards_i, \gamma_i, \pi_i)$.
%
%Here, $\pi_i$ is the agent's policy.
%
For the \tom approaches we shall assume access to (potentially partial and/or noisy)
observations of the agents, via a state-observation function
$\stateobsfun(\cdot) : \states \rightarrow \Omega^{\obs}$
and an action-observation function
$\actionobsfun(\cdot) : \actions \rightarrow \action^{\obs}$.
%
For each agent $\agents_i$ in a POMG $\M_j$ we assume our observer
can see $\tauobs_{i,j} = \{(\stateobs, \actionobs)\}^{T}_{t=0}$,
where $\actionobs = \actionobsfun(a_t)$ and $\stateobs = \stateobsfun(s_t)$.
%
%Similar to the
%original \tomnet paper~\cite{pmlr-v80-rabinowitz18a},
%we associate the reward functions, discount factors,
%and conditional observation functions with the agents rather
%than the POMG.
%
%For the \tom approaches we shall assume access to (potentially partial and/or noisy)
%observations of the agents, via a state-observation function
%$\stateobsfun(\cdot) : \states \rightarrow \Omega^{\obs}$
%and an action-observation function
%$\actionobsfun(\cdot) : \actions \rightarrow \action^{\obs}$.
%
%For each agent $A_i$ in a POMG $\M_j$, we assume our observer
%can see $\tau_{ij}^{\obs} = \{(\stateobs, \actionobs)\}^{T}_{t=0}$,
%where $\actionobs = \actionobsfun(a_t)$ and
%$\stateobs = \stateobsfun(s_t)$.
%
Critically, setting $\stateobsfun(\cdot)$
and $\actionobsfun(\cdot)$ to the identity function grants the observer
unrestricted access to the POMG state along with all overt actions taken
by the agents while keeping their parameters,
reward functions, policies, and identifiers concealed.
%
This formulation closely approximates the depth of knowledge
that would be available to a human observer in a real-world
scenario.

Our approaches are based on the original \tomnet from \cite{rabinowitz2018machine},
depicted in \autoref{fig:ToM}.
%
To recap, \tomnet consists of three modules, a
\emph{character net},
\emph{mental net}, and
a \emph{prediction net}.
%
The character net $f_{\theta}$ yields a character embedding
$\characteri$ upon parsing $n$ past trajectories $\tauobs$
for an agent $\agents_i$, $\{\tauobs_{i,j}\}^{N_{past}}_{j=1}$.
%
As in the original paper, we shall process the
trajectories independently using a
recurrent neural network,
specifically a Long Short-Term Memory (LSTM) network \cite{hochreiter1997long}
$f_\theta$, and sum the outputs:
%
\begin{equation} \label{eq:characteri}
\characteri = \sum^{N_{past}}_{j=1}f_\theta \Bigbrackets{\tauobs_{ij}}.
\end{equation}
%
The mental (state) net $g_{\vartheta}$ meanwhile processes the current
trajectory up to time-step $t-1$ along with $\characteri$:
%
\begin{equation}
\mentali = g_{\vartheta}\Bigbrackets{[\tauobs_{ij}]_{0:t-1}, \characteri}.
\end{equation}
%
The prediction net subsequently uses both embeddings and the current
state $\state$ to predict the agent's behaviour, including: The policy
$\hat{\pi}(\cdot \rvert \state^{\obs}_t, \characteri, \mentali)$; items
that the agent will consume $\hat{c}$ (\eg a high value target node that
a \red cyber-attacking agent wants to gain access to), and; the successor
representations $\SR$, the expected discounted state occupancy
% ~\citep{dayan1993improving}.

\subsection{Summary}

In this section we outlined the definitions and notations that we shall
use in this report.
%
We formally define the environments that our cyber-defence and attacking
agents inhabit as partially observable Markov games, and provided a recap of the
original \tomnet architecture.
%
Next we shall take a closer look at our problem formulation.

